First-Order Adaptive Sample Size Methods to Reduce Complexity of Empirical Risk Minimization

This paper studies empirical risk minimization (ERM) problems for large-scale datasets and incorporates the idea of adaptive sample size methods to improve the guaranteed convergence bounds for first-order stochastic and deterministic methods. In contrast to traditional methods that attempt to solve the ERM problem corresponding to the full dataset directly, adaptive sample size schemes start with a small number of samples and solve the corresponding ERM problem to its statistical accuracy. The sample size is then grown geometrically -- e.g., scaling by a factor of two -- and use the solution of the previous ERM as a warm start for the new ERM. Theoretical analyses show that the use of adaptive sample size methods reduces the overall computational cost of achieving the statistical accuracy of the whole dataset for a broad range of deterministic and stochastic first-order methods. The gains are specific to the choice of method. When particularized to, e.g., accelerated gradient descent and stochastic variance reduce gradient, the computational cost advantage is a logarithm of the number of training samples. Numerical experiments on various datasets confirm theoretical claims and showcase the gains of using the proposed adaptive sample size scheme.

==> localnewton.tex <==
%!TEX root = adap-ss-nips.tex

\section{Algorithm and Analysis}

We suggest to modify Newton's method to work with a dynamic sample size schedule. We here further assume that the loss function $f_\x(\w)$ - and therefore the risk function $\risk_\S(\w)$ - are self-concordant functions~\cite{nesterov1994interior}. Formally, $f_\x(\w)$ is self-concordant if it is convex and if
\begin{equation}
|\nabla^3 f_\x(\w)| \leq 2 \nabla^2 f_\x(\w)^{3/2}.
\end{equation}
The last condition implies that the rate of change in curvature of $f$ is bounded by the curvature which is true of linear and quadratic functions. This concept has also be generalized to apply to the logistic loss function in~\cite{bach2010self}.

\subsection{Newton's method}

We here focus on the analysis for self-concordant functions which is very similar to the classical analysis based on strong-convexity except that the Newton decrement will play the role of the norm of the gradient. The convergence rate of Newton's method is characterized by a phase transition between two different regimes~\cite{boyd04}. As the estimate is still far away from the optimum, we observe a "global" phase characterized by a sublinear rate. This phase typically requires a line search procedure to determine a good step-size for each step. This procedure is in practice very expensive as it requires evaluating the loss function $f_\x(\w)$ at various points around the current estimate $\w$. As the estimate gets close to the optimum solution, Newton's method enters a local phase for which the convergence rate becomes quadratic.

The two-phase regime of Newton's method is summarized in the following lemma.

\begin{lemma}[\textbf{Newton's Convergence Rate}]
\label{lemma:newton_convergence} 
	Define $\lambda(\w)$ as:
	\begin{equation} \label{eq:locality_measure}
		\lambda(\w) = \left[ \nabla^T \risk (\w) \nabla^2 \risk(\w)^{-1}
	\nabla \risk(\w) \right]^{1/2},
	\end{equation}
	and assume there exists a constant $\eta \in [0, 1/4]$~\footnote{$\eta$ is a constant that depends on line search parameters. We refer the reader to~\cite{boyd04} for further details.}.
	The convergence rate of Newton's convergence includes two phases : 
	\begin{itemize}
	  \item[a.] ``Global phase'': if $\lambda(\w)> \eta$, then
	  \begin{equation}
	  		\risk_\S(\w^+) - \risk_\S(\w) \leq - \gamma
	  \end{equation}
	  where $\gamma < 1$ is a constant
	  parameter depends on line search parameters.
	  \item[b.] ``Local phase'': if $\lambda(\w) < \eta$ then
	    \begin{equation}
	    	 \risk_\S(\w^+)- \risk_\S^* \leq 24 \left(\risk_\S(\w) - \risk_\S^*
		 \right)^2
	    \end{equation}
	\end{itemize} 
	\begin{proof}
	    The convergence of the \textit{global phase} is proved in
	    \cite{nesterov2004introductory}.
	    A convergence proof for the \textit{local phase} is given in Lemma~\ref{lemma:quadratic_risk}, where we use the bound of~\cite{nesterov2004introductory} derived in terms of $\lambda(\w)$ and translate it in terms of risk value.
	\end{proof}
\end{lemma}

 Using the above result, one can easily show that the total number of
 iterations required to obtain an $(\epsilon,\S)$-optimal solution is bounded by
\begin{equation}
	\frac{\risk_\S (\w^0) - \risk_{\S}^*}{ \gamma} + \log_2 \log_2
	(1/\epsilon).
\end{equation} 


\subsection{Newton's method with adaptive sample size}
\label{sec:dyna_newton}

\highlight{aurelien: currently editing this part}

\comment{
The previous analysis suggests that one could significantly speed-up the convergence speed of Newton's method by entering the local phase.
}

As the above equation shows, the main challenge of Newton's is passing the
global region. Indeed, computational complexity of global phase linearly depends
on the initial error $\risk_\S (\w^0) - \risk_{\S}^*$.
Here, the main challenge is number of required steps to reach the local neighbourhood that has
a linear dependency to the initial error $\risk_\S(\w^0) - \risk_{\S}^*$.

We here suggest accelerating Newton's method using the following idea. We start optimizing on a small set $\S$, then add samples to $\S$ while reducing the regularizer (as $1/|\S|$) such that the current estimate $\w$ always lies in the local region of the enlarged set. One compelling argument of such a technique is that it suppresses the need for an expensive line search procedure while also reducing the number of gradient evaluations. Each iteration of Newton method takes $\bigO(n d^2 + d^3)$ on set $|\S| = n$. In our setting, where $n \gg d$ the iteration complexity is limited by size of the set, i.e. is $\bigO(n d^2)$. Hence, a smaller set $| \T | = m$ imposes
$m/n$-factor of improvement in computational complexity. In this case, we say
iteration on the smaller set takes $m/n$-pass over the training set $\S$. Using
this fact, next Proposition states the required passes over the training set to
obtain $(\epsilon,\S)$-optimality.

Algorithm~\ref{alg:localnewton} represents details of \localnewton.\\ 


%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[tb]
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} \\
   $\quad$ training examples $\S = (\x_1,\x_2,\ldots,\x_n)$, $\x_i \sim P$\\
   $\quad$ initial set $\T \subset \S$, where $|T| = m_0$ and $m_0$ is chosen
   according to Corollary~\ref{cor:initial_sample_size}. \\
   $\quad$ initial iteration number $T_0$ according to
   Equation~\ref{eq:initial_steps}. \\
   $\quad$ starting point $\w_0 \in \mbR^d$\\
%   \STATE {\bfseries Initialization:} \\
   \STATE $\w \leftarrow \w_0$
   \STATE $M \leftarrow m_0$ \highlight{ -- consider changing this to $m$ to be consistent with the text}
   \FOR{$k=1,\dots,K$}
   \IF{$M = m_0$}
   	 \STATE $T \leftarrow T_0$
   \ELSE
    \STATE $T \leftarrow 1$
   \ENDIF
   \FOR{$t=1,\dots,T$}
   	   \STATE sample $\T \leftarrow (\x_1,\dots,\x_{M})$
	   \STATE $g \leftarrow \nabla \risk_\T(\w_{t-1})$
	   \STATE $H \leftarrow  \nabla^2 \risk_\T(\w_{t-1})$ 
	   \STATE $\w_t \leftarrow \w_{t-1} - H^{-1} g$
   \ENDFOR
   \STATE $M \leftarrow 2M$
   \STATE $\w \leftarrow \w_T$
   \ENDFOR
\end{algorithmic}
\caption{{\localnewton}}
\label{alg:localnewton}
\end{algorithm}
\begin{lemma}[Convergence Gaurantee] \label{lemma:localnewton_convergence}
	Given $\bound(n) = D/n$, a training set $\S$ of size $|\S | = n $, $L \leq \eta^2/(4D + \| \w^* \|^2)$, then \localnewton guarantees
	$(n^{-2^{(k-1)}},\S)$-optimality after $k+1+ \delta$ passes over the data, where
	\begin{equation}
		\delta = \frac{m_0}{n} \left(\frac{\risk_\S(\w_0)-\risk_\S^*+4}{\gamma} + 1
		\right)
	\end{equation}
	and $m_0$ is determined by Corollary~\ref{cor:initial_sample_size}. 
	\begin{proof}
	    \highlight{Need to simplify this!} We provide a bound on initial error on $\T$, i.e. $\risk_\T(\w)-
	    \risk_\T^*$, using the initial error on the main training set $\S$. 
	    According to corollary~\ref{cor:initial_sample_size},
	    $(1/m_0^2,\T)$-optimality is guaranteed after $T_0$ iterations (defined in
	    Equation~\ref{eq:initial_steps}).
	    Computationally, this would be equivalent to $\delta = T_0/n$ passes over the training set $| \S | = n$.
		Then, Lemma~\ref{lemma:doubling_for_locality} insures that parameters lies
		in the local neighbourhood of the enlarged set. On the enlarged set, one
		iteration suffices to decrease $(1/m,\T)$-optimality --of the local
		neighbourhood-- to $(1/m^2,\T)$-optimality that is againe required by the
		locality condition for the next step. It easy to show that \textit{doubling}
		phase computationally takes at most one pass over the data and then we lie in local
		neighbourhood of the main set $\S$. In other words, after $1 + \delta$ passes $(1/n,\S)$-optimality
		obtains, hence the rate $(n^{-2^{(k-1)}},\S)$-optimality is guaranteed by
		quadratic convergence rate of the Newton's method.
	\end{proof}
\end{lemma}
\begin{remark}
	In the setting where large scale setting when 
	\begin{equation}
	\frac{m_0}{\gamma} \left(\risk_\S(\w_0) - \risk_\S^*\right) < n,
	\end{equation}
	the $\delta$ is less than one passes over the data. According to
	Lemma~\ref{lemma:localnewton_convergence}, \localnewton needs constant
	number of passes to obtain arbitrary accurate solution, which is
	completely independent of the initial error. However, Newton's method theoretically requires
	at least $\gamma^{-1}\left(\risk_\S(\w_0) - \risk_\S^*\right)$-passes over the
	data~\cite{boyd04}.
\end{remark}
